DisCor: Corrective Feedback in Reinforcement Learning via Distribution Correction

Deep reinforcement learning can learn effective policies for a wide range of tasks, but is notoriously difficult to use due to instability and sensitivity to hyperparameters. The reasons for this remain unclear. When using standard supervised methods (e.g., for bandits), on-policy data collection provides "hard negatives" that correct the model in precisely those states and actions that the policy is likely to visit. We call this phenomenon "corrective feedback." We show that bootstrapping-based Q-learning algorithms do not necessarily benefit from this corrective feedback, and training on the experience collected by the algorithm is not sufficient to correct errors in the Q-function. In fact, Q-learning and related methods can exhibit pathological interactions between the distribution of experience collected by the agent and the policy induced by training on that experience, leading to potential instability, sub-optimal convergence, and poor results when learning from noisy, sparse or delayed rewards. We demonstrate the existence of this problem, both theoretically and empirically. We then show that a specific correction to the data distribution can mitigate this issue. Based on these observations, we propose a new algorithm, DisCor, which computes an approximation to this optimal distribution and uses it to re-weight the transitions used for training, resulting in substantial improvements in a range of challenging RL settings, such as multi-task learning and learning from noisy reward signals. Blog post presenting a summary of this work is available at: https://bair.berkeley.edu/blog/2020/03/16/discor/.

==> sections/05_1_derivation.tex <==
\section{Theoretical Derivation of DisCor}
\label{sec:theoretical_derivation}
In this section, we present a sketch of the theoretical derivation of the DisCor algorithm (Algorithm~\ref{alg:discor}) from the perspective of maximizing corrective feedback, $\valuefeedback$. We present an optimization problem for the optimal data distribution, and then discuss how to solve this optimization problem in Section~\ref{sec:objective_derivation}. These derivations assume access to the optimal Q-function $Q^*$, as well as future Q-functions $Q_{l}$ that will be encountered in Q-learning. Finally, in Section~\ref{sec:minimax}, we justify the choice of $\Delta_k$ as an estimator for \mbox{$|Q_k - Q^*|$}, bridging the gap between theory and practice. The complete derivation is provided in Appendix~\ref{sec:missing_proof_steps}. 




\subsection{From Corrective Feedback to a Tractable Optimization Problem}
\label{sec:objective_derivation}
Our goal is to maximize the value of corrective feedback $\valuefeedback(k)$ at every iteration $k$, with respect to the the $p_k$ used for Bellman error minimization at iteration $k$. 
Since $Q_{k-1}$ does not depend on the choice of $p_k$ and is known beforehand, we disregard the term dependent on $Q_{k-1}$, and only optimize the term dependent on $Q_k$. 
The resulting optimization problem is:
\begin{multline}
    \vspace{-10pt}
    \quad \min_{p_k}~~ \expec_{d^{\pi_{k}}} \left[ |Q_k - Q^*| \right] \\
    \text{~~s.t.~~} Q_k = \arg\min_{Q} \expec_{p_k} \left[ (Q - \bellmanopt Q_{k-1})^2 \right]. 
    \label{eqn:optimization}
\end{multline}
The key steps in the derivation are sketched below and described in detail in Appendix~\ref{sec:missing_proof_steps}. Since the optimization objective is the inner product of $d^{\pi_{k-1}}$ and $|Q_k - Q^*|$, we decompose this objective by applying the Fenchel-Young inequality~\cite{rockafellar-1970a}, which states for any two vectors, $x, y \in \mathbb{R}^d$, and any convex function $f$ and its Fenchel conjugate $f^*$, $x^T y \leq f(x) + f^*(y)$. 
\begin{equation}
    \label{eqn:convex_conjugate}
    \expec_{d^{\pi_k}} \left[ |Q_k - Q^*| \right] \leq f\left( |Q_k - Q^*| \right) + f^* \left( d^{\pi_k} \right).
\end{equation} 
A convenient choice of $f$ is the \emph{soft-min} function:
\begin{equation}
    f(x) = - \log \big( \sum_{i} e^{-x_i} \big), ~~ f^*(y) = \mathcal{H}(y).
    \label{eqn:f_and_conjugate}
    \vspace{-10pt}
\end{equation}
The additional entropy term $\mathcal{H}(d^{\pi_k})$ introduced via the application of Fenchel-Young inequality is upper bounded by the entropy of the uniform distribution, $\mathcal{H}(\mathcal{U})$, such that
\begin{equation}
    \label{eqn:f_with_entropy}
    \expec_{d^{\pi_k}} \left[ |Q_k - Q^*| \right] \leq f(|Q_k - Q^*|) + \mathcal{H}(\mathcal{U}). 
\end{equation}
We then minimize the upper bound shown in Equation~\ref{eqn:f_with_entropy}. As we will note in Appendix~\ref{sec:missing_proof_steps}, the upper bound step in Equation~\ref{eqn:f_with_entropy} can also be interpreted as encouraging exploration in $\pi_k$ by providing it an intrinsic motivation bonus, or as smoothing the objective landscape~\cite{ahmed19understanding}. Thus, the final optimization problem is:
\begin{multline}
    \label{eqn:final_optimization}
    \vspace{-10pt}
    \min_{p_k}~~~ - \log \left( \sum_{s, a} \exp({- |Q_k - Q^*|(s, a)}) \right) \\
    \text{~~s.t.~~} Q_k = \arg\min_{Q} \expec_{p_k} \left[ (Q - \bellmanopt Q_{k-1})^2 \right]
\end{multline}
In order to derive the solution of Problem~\ref{eqn:final_optimization}, we follow standard procedures of computing the Lagrangian, and applying KKT conditions~\cite{}.
We present a detailed derivation in Appendix~\ref{sec:missing_proof_steps}.
The optimal $p_k(s, a)$, expressed in terms of the optimal dual variable $\lambda^* \in \mathbb{R}^{+}$
is given by:
\begin{equation}
    \label{eqn:optimal_p}
    \vspace{-3pt}
    p_k(s, a) \propto \exp\left(-|Q_k - Q^*|(s, a)\right) \frac{|Q_k - \bellmanopt Q_{k-1}|(s, a)}{\lambda^*}
\end{equation}
DisCor reweights transitions drawn from the replay buffer distribution, $\mu(s, a)$ via importance sampling. A na\"ive application of importance sampling $w_k(s, a) = \frac{p_k(s, a)}{\mu(s, a)}$ results in high-variance importance weights. To prevent thos, we instead reweight to a projection of $p_k$ that keeps it close to the buffer distribution $\mu$.
More details are provided in Appendix~\ref{sec:missing_proof_steps}, Step 5. Thus, the final form for $w_k$ is given by:
\begin{equation}
    \label{eqn:optimal_wk}
    \vspace{-3pt}
    w_k(s, a) \!\propto\! \exp\!\left(\!\frac{-|Q_k - Q^*|(s, a)}{\tau}\!\right)\! \frac{|Q_k - \bellmanopt Q_{k-1}|(s, a)}{\lambda^*}
\end{equation}
where $\tau$ is a temperature hyperparameter. Intuitively, the expression in Equation~\ref{eqn:optimal_wk} assigns higher probability to state-action tuples with high Bellman error $|Q_k - \bellmanopt Q_{k-1}|$, but only when the resulting Q-value $Q_k$ is close to $Q^*$. {This is consistent with the DisCor Algorithm -- $w_k$ minimizes Bellman error on only those transitions which lead to more corrective updates, i.e. have a smaller \mbox{$|Q_k - Q^*|$}, after the Q-function update.} In order to derive DisCor from here, we need a way to estimate $|Q_k - Q^*|$ as the final piece.


\subsection{Tractably Estimating $|Q_k - Q^*|$}
\label{sec:minimax}
The expression for $w_k$ in Equation~\ref{eqn:optimal_wk} contains terms that depend on $Q^*$. Since both $Q_k$ and $Q^*$ are observed only \emph{after} $w_k$ is chosen, we need to estimate these quantities. In Section~\ref{sec:method_description} we used the cumulative sum of discounted Bellman errors $\Delta_k$ over the past iterations of training as a proxy for this term, $|Q_k - Q^*|$. Here we show that $\Delta_k$ is indeed a theoretically justified choice, as a tractable upper bound on $|Q_k - Q^*|$ constructed only from prior Q-function iterates, $Q_0, \cdots, Q_{k-1}$. {A upper bound of this form may downweight transitions with accurate target values, but would never upweight transitions with inaccurate target values.}
\begin{lemma}
\label{thm:worst_case_estimator}
For any $k \in \mathbb{N}$, $|Q_k - Q^*|$ satisfies the following recursive inequality, pointwise for each $s, a$:
\begin{multline*}
|Q_k - Q^*| \leq |Q_k - \bellmanopt Q_{k-1}| +\\ \gamma P^{\pi_{k-1}} |Q_{k-1} - Q^*| + \frac{2 R_{\text{max}}}{1 - \gamma} \max_{s} \tvd(\pi_{k-1}, \pi^*).    
\end{multline*}
\end{lemma}
We now derive an estimator, which corresponds to the quantity denoted $\Delta_k(s, a)$ in the DisCor algorithm, using this inequality.
{This estimator is the solution of the recursive equation corresponding to the recursive inequality in Lemma~\ref{thm:worst_case_estimator}, offset by a state-independent constant $\max_{s} \tvd(\pi_{k-1}, \pi^*)$ for each $k$. In fact, we can show that $\Delta_k$ satisfies $\Delta_k + \sum_i \gamma^i \alpha_i \geq |Q_k - Q^*|$ pointwise, for a sufficiently large $k$, where $\alpha_k = \max_{s} \tvd(\pi_k, \pi^*)$ is a scalar, constant across any state-action pair, and goes to $0$ as $k$ increases, thus making $\Delta_k$ a tighter approximation to $|Q_k - Q^*|$ as $k$ increases. We formally prove this in Appendix~\ref{sec:missing_proof_steps}, Theorem~\ref{thm:alpha}. Thus, we can use $\Delta_k$ directly to choose a weighting.}

We finally note that the expression for $w_k$ in Equation~\ref{eqn:importance_weights} does not include the Bellman error term, $|Q_k - \bellmanopt Q_{k-1}|$, like in Equation~\ref{eqn:optimal_wk}, and uses an estimate of error propagated from the target value, $P^{\pi_{k-1}} \Delta_{k-1}$, instead of $\Delta_k$. This is because the term $|Q_k - \bellmanopt Q_{k-1}|$ is unknown, since $Q_k$ is not known when $w_k$ is chosen. Instead $Q_k$, is the result of Bellman error minimization with weights $w_k$. With no available information about $Q_k$, a worst-case bound upper bounds for $|Q_k - \bellmanopt Q_{k-1}|$ is a constant, and hence we get Equation~\ref{eqn:importance_weights} from Equation~\ref{eqn:optimal_wk}.





==> sections/5_method_new.tex <==
\section{Distribution Correction (DisCor)}
\label{sec:method_description}
Based on the observations in the previous section, we propose a method for modifying the training distribution that explicitly optimizes for corrective feedback. At each iteration $k$ of the ADP algorithm, our method aims to select the distribution $p_k(\s,\mathbf{a})$ such that training under this distribution maximizes corrective feedback.
We will present a theoretical derivation of our method as explicit optimization of corrective feedback in Section~\ref{sec:theoretical_derivation}, while in this section we describe the method along with a more intuitive explanation.
Intuitively, our method chooses $p_k$ so as to \textit{downweight} those transitions for which the bootstrapped \emph{target} Q-value has a high estimated error to $Q^*$. This way, backups are only performed on accurate target values, effectively resulting in no error accumulation, thus ensuring correct feedback. This resembles prior methods for training with noisy labels, which aim to achieve lower empirical risk and better generalization by ``abstention'' from training on labels that are likely to be inaccurate~\cite{absention}.

In order to train only on transitions with target values that have a small error to $Q^*$, we need to estimate $|Q_k - Q^*|$ using a surrogate estimator, since this quantity is unknown because $Q^*$ itself is unknown. Our method uses  the cumulative sum of discounted Bellman errors over previous iterations of training, $0, \cdots, k-1$, to approximate this quantity. We refer to this term as $\Delta_k$ in Equation~\ref{eqn:delta_k}. As we will argue in Section~\ref{sec:minimax}, this represents a tractable upper bound for $|Q_k - Q^*|$, and this bound becomes tight as the learned policy approaches the optimal policy. A worst-case upper bound $\Delta_k$ may downweight transitions that have accurate target values, but would never upweight transitions with inaccurate target values. Formally, $\Delta_k$ is given by
\vspace{-15pt}
\begin{multline}
\Delta_k = \sum_{i=1}^{k-1} \gamma^{k-i} \left(\prod_{j=i+1}^{k-1} P^{\pi_{j}} \right) |Q_{i} - \bellmanopt Q_{i-1}| \\
   \implies  \Delta_k = |Q_k - \bellmanopt Q_{k-1}| + \gamma P^{\pi_{k-1}} \Delta_{k-1} .
    \label{eqn:delta_k}
\vspace{-15pt}
\end{multline}
Having calculated $\Delta_k$, we can utilize it to reweight the transitions that have already been collected in a replay buffer, and combine it with any ADP method. Pseudocode for this approach, which we call \textbf{DisCor} (\textbf{Dis}tribution \textbf{Cor}rection), is presented in Algorithm~\ref{alg:discor}, with the main differences from standard ADP methods highlighted in red. In addition to a standard Q-function, DisCor trains another parametric model, $\Delta_\phi$, to estimate $\Delta_k(s, a)$ at each state-action pair. The recursion in Equation~\ref{eqn:delta_k} is used to obtain a simple approximate dynamic programming update rule for the parameters $\phi$ (Line 8).
The second change is the introduction of a weighted Q-function backup with weights $w_k(s, a)$, on Line 7. This corresponds to using importance sampling to train on the distribution $p_k$ while only having access to buffer samples.
The formula for these weights based on the discussion so far, which we also will derive more formally in Section~\ref{sec:theoretical_derivation}, is given by:
\begin{equation}
    w_k \propto \exp{\left(-\frac{\gamma P^{\pi_{k-1}} \Delta_{k-1}}{\tau} \right)} %
    \label{eqn:importance_weights}
\end{equation}
Here, $P^{\pi_{k-1}} \Delta_{k-1}$ corresponds to the estimated upper bound on the error of the target values for the current transition, due to the backup operator $P^{\pi_{k-1}}$. This means that transitions with erroneous targets are downweighted, 
effectively focusing the learning on samples where the supervision (target value) is accurate, 
which are precisely the samples that we expect maximally improve the accuracy of the Q function.

\begin{algorithm}[t]
\small
\caption{\textbf{DisCor (Distribution Correction)}}
\label{alg:discor}
\begin{algorithmic}[1]
    \STATE Initialize Q-values $Q_\theta(s, a)$, initial distribution $p_0(s, a)$, a replay buffer $\beta$, and an \textdiff{error model} $\Delta_\phi(s, a)$.
    \FOR{step $k$ in \{1, \dots, N\}}
        \STATE Collect $M$ samples using $\pi_k$, add them to replay buffer $\beta$, sample $\{(s_i, a_i)\}_{i=1}^N \sim \beta$
        \STATE Evaluate $Q_\theta(s,a)$ and $\Delta_\phi(s, a)$ on samples $(s_i, a_i)$.
        \STATE Compute target values for $Q$ and $\Delta$ on samples:\\
        ${y}_i = r_i + \gamma \max_{a'} Q_{k-1}(s'_i, a')$\\ $\hat{a}_i = \arg \max_{a} Q_{k-1}(s'_i, a) $\\
        $\hat{\Delta}_{i} = |Q_\theta(s, a) - y_i| + \gamma \Delta_{k-1}(s'_i, \hat{a}_i)$
        \STATE \textdiff{Compute $w_k$ using Equation~\ref{eqn:importance_weights}}. 
        \STATE Minimize Bellman error for training $Q_\theta$ weighted by $w_k$. \\
        $ \theta_{k+1} \leftarrow \argmin{\theta} \frac{1}{N}\sum_{i=1}^N \textdiff{w_k(s_i, a_i)} \cdot (Q_\theta(s_i,a_i) - y_i)^2$
        \STATE \textdiff{Minimize ADP error for training $\phi$. \\
        $\phi_{k+1} \leftarrow \argmin{\phi} \frac{1}{N} \sum_{i=1}^N (\Delta_\theta(s_i, a_i) - \hat{\Delta}_i)^2$}
    \ENDFOR
\end{algorithmic}
\end{algorithm}
Next, we present a theoretical derivation of the DisCor algorithm starting from the problem of maximizing value of corrective feedback, $\valuefeedback$, and reducing it to the choice of the distribution/weights for minimizing Bellman error.  























